5-Coloring Reconfiguration of Planar Graphs with No Short Odd Cycles

The coloring reconfiguration graph $\mathcal{C}_k(G)$ has as its vertex set all the proper $k$-colorings of $G$, and two vertices in $\mathcal{C}_k(G)$ are adjacent if their corresponding $k$-colorings differ on a single vertex. Cereceda conjectured that if an $n$-vertex graph $G$ is $d$-degenerate and $k\geq d+2$, then the diameter of $\mathcal{C}_k(G)$ is $O(n^2)$. Bousquet and Heinrich proved that if $G$ is planar and bipartite, then the diameter of $\mathcal{C}_5(G)$ is $O(n^2)$. (This proves Cereceda's Conjecture for every such graph with degeneracy 3.) They also highlighted the particular case of Cereceda's Conjecture when $G$ is planar and has no 3-cycles. As a partial solution to this problem, we show that the diameter of $\mathcal{C}_5(G)$ is $O(n^2)$ for every planar graph $G$ with no 3-cycles and no 5-cycles.

==> pgflibrarybbox.code.tex <==
\tikzset{%
  bezier bounding box/.is choice,%
  bezier bounding box/.default=true,%
  bezier bounding box/true/.code=\tikzset{switch on bezier bounding box},%
  bezier bounding box/false/.code=\tikzset{switch off bezier bounding box}}%
\tikzset{switch off bezier bounding box/.code={%
\def\pgf@lt@curveto##1##2##3##4##5##6{%
  \pgf@protocolsizes{##1}{##2}%
  \pgf@protocolsizes{##3}{##4}%
  \pgf@protocolsizes{##5}{##6}%
  \pgfsyssoftpath@curveto{\the##1}{\the##2}{\the##3}{\the##4}{\the##5}{\the##6}%
}%
\let\pgf@nlt@curveto\pgf@lt@curveto}}
%
% it might just be me but according to what I believe to find 
% \pgfmathsetlengthmacro appears to generate spaces
%
\tikzset{switch on bezier bounding box/.code={%
\def\pgf@lt@curveto##1##2##3##4##5##6{%
  % extrema in x
  \pgfmathsetmacro{\pgf@temp@b}{abs(\pgf@path@lastx-##5-3*##1+3*##3)}%
  % ^^^ this is used for the denominator below, cannot become too small
  \pgfmathsetmacro{\pgf@temp@c}{max(1+\pgf@path@lastx,max(##1,max(##3,##5)))}%
  % ^^^ in order to avoid dimension too large errors from squaring lengths in pt
  \pgfmathparse{((##1/\pgf@temp@c)*(##1/\pgf@temp@c)-1*((##1/\pgf@temp@c)*(##3/\pgf@temp@c))+(##3/\pgf@temp@c)*(##3/\pgf@temp@c)-1*((##1/\pgf@temp@c)*(##5/\pgf@temp@c))+(-(##3/\pgf@temp@c)+(##5/\pgf@temp@c))*(\pgf@path@lastx/\pgf@temp@c))}%
  \pgfutil@tempdima=\pgfmathresult pt\relax% 
  % ^^^ discriminant
  \ifdim\pgf@temp@b pt<0.01pt\relax%
   % approximately linear  
   \pgfmathparse{abs(2*(##1)-2*(##3)+(##5))}%
   \pgfutil@tempdimb=\pgfmathresult pt\relax%
   \ifdim\pgfutil@tempdimb<0.1pt\relax%
    % if the denominator is very small, it is *likely* large but could be 0/0
   \else
    \pgfmathsetmacro{\pgf@temp@a}{(2*(##1)-3*(##3)+(##5))/(2*(##1)-2*(##3)+(##5))}%
    \pgfmathparse{\pgf@path@lastx*pow(1-\pgf@temp@a,3)+3*##1*pow(1-\pgf@temp@a,2)*\pgf@temp@a+3*##3*(1-\pgf@temp@a)*\pgf@temp@a*\pgf@temp@a+##5*pow(\pgf@temp@a,3)}%
    \pgfutil@tempdimb=\pgfmathresult pt\relax%
    \pgf@protocolsizes{\pgfutil@tempdimb}{##6}%
   \fi%
  \else
   \ifdim\pgfutil@tempdima<0pt\relax% negative discriminant -> no turning point
   \else
     \pgfmathsetmacro{\pgf@temp@a}{min(1,max(0,(\pgf@path@lastx-2*##1+##3-\pgf@temp@c*sqrt(\pgfutil@tempdima))/(\pgf@path@lastx-##5-3*##1+3*##3)))}%
     \pgfmathparse{\pgf@path@lastx*pow(1-\pgf@temp@a,3)+3*##1*pow(1-\pgf@temp@a,2)*\pgf@temp@a+3*##3*(1-\pgf@temp@a)*\pgf@temp@a*\pgf@temp@a+##5*pow(\pgf@temp@a,3)}%
     \pgfutil@tempdimb=\pgfmathresult pt\relax%
     \pgf@protocolsizes{\pgfutil@tempdimb}{##6}%
     \pgfmathsetmacro{\pgf@temp@a}{min(1,max(0,(\pgf@path@lastx-2*##1+##3+\pgf@temp@c*sqrt(\pgfutil@tempdima))/(\pgf@path@lastx-##5-3*##1+3*##3)))}%
     \pgfmathparse{\pgf@path@lastx*pow(1-\pgf@temp@a,3)+3*##1*pow(1-\pgf@temp@a,2)*\pgf@temp@a+3*##3*(1-\pgf@temp@a)*\pgf@temp@a*\pgf@temp@a+##5*pow(\pgf@temp@a,3)}%
     \pgfutil@tempdimb=\pgfmathresult pt\relax%
     \pgf@protocolsizes{\pgfutil@tempdimb}{##6}%
   \fi% 
  \fi 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  % extrema in y (completely analogous to the above)
  \pgfmathsetmacro{\pgf@temp@b}{abs(\pgf@path@lasty-##6-3*##2+3*##4)}%
  \pgfmathsetmacro{\pgf@temp@c}{max(1+\pgf@path@lasty,max(##2,max(##4,##6)))}%
  \pgfmathparse{((##2/\pgf@temp@c)*(##2/\pgf@temp@c)-1*((##2/\pgf@temp@c)*(##4/\pgf@temp@c))+(##4/\pgf@temp@c)*(##4/\pgf@temp@c)-1*((##2/\pgf@temp@c)*(##6/\pgf@temp@c))+(-(##4/\pgf@temp@c)+(##6/\pgf@temp@c))*(\pgf@path@lasty/\pgf@temp@c))}%
  \pgfutil@tempdima=\pgfmathresult pt\relax% 
  % ^^^ discriminant
  \ifdim\pgf@temp@b pt<0.01pt\relax%
   % approximately linear  
   \pgfmathparse{abs(2*(##2)-2*(##4)+(##6))}%
   \pgfutil@tempdimb=\pgfmathresult pt\relax%
   \ifdim\pgfutil@tempdimb<0.1pt\relax%
    % if the denominator is very small, it is *likely* large but could be 0/0
   \else
    \pgfmathsetmacro{\pgf@temp@a}{(2*(##2)-3*(##4)+(##6))/(2*(##2)-2*(##4)+(##6))}%
    \pgfmathparse{\pgf@path@lasty*pow(1-\pgf@temp@a,3)+3*##2*pow(1-\pgf@temp@a,2)*\pgf@temp@a+3*##4*(1-\pgf@temp@a)*\pgf@temp@a*\pgf@temp@a+##6*pow(\pgf@temp@a,3)}%
    \pgfutil@tempdimb=\pgfmathresult pt\relax%
    \pgf@protocolsizes{##5}{\pgfutil@tempdimb}%
   \fi%
  \else
   \ifdim\pgfutil@tempdima<0pt\relax% negative discriminant -> no turning point
   \else
     \pgfmathsetmacro{\pgf@temp@a}{min(1,max(0,(\pgf@path@lasty-2*##2+##4-\pgf@temp@c*sqrt(\pgfutil@tempdima))/(\pgf@path@lasty-##6-3*##2+3*##4)))}%
     \pgfmathparse{\pgf@path@lasty*pow(1-\pgf@temp@a,3)+3*##2*pow(1-\pgf@temp@a,2)*\pgf@temp@a+3*##4*(1-\pgf@temp@a)*\pgf@temp@a*\pgf@temp@a+##6*pow(\pgf@temp@a,3)}%
     \pgfutil@tempdimb=\pgfmathresult pt\relax%
     \pgf@protocolsizes{##5}{\pgfutil@tempdimb}%
     \pgfmathsetmacro{\pgf@temp@a}{min(1,max(0,(\pgf@path@lasty-2*##2+##4+\pgf@temp@c*sqrt(\pgfutil@tempdima))/(\pgf@path@lasty-##6-3*##2+3*##4)))}%
     \pgfmathparse{\pgf@path@lasty*pow(1-\pgf@temp@a,3)+3*##2*pow(1-\pgf@temp@a,2)*\pgf@temp@a+3*##4*(1-\pgf@temp@a)*\pgf@temp@a*\pgf@temp@a+##6*pow(\pgf@temp@a,3)}%
     \pgfutil@tempdimb=\pgfmathresult pt\relax%
     \pgf@protocolsizes{##5}{\pgfutil@tempdimb}%
   \fi% 
  \fi 
  \pgf@protocolsizes{\pgf@path@lastx}{\pgf@path@lasty}%
  \pgf@protocolsizes{##5}{##6}%
  \pgfsyssoftpath@curveto{\the##1}{\the##2}{\the##3}{\the##4}{\the##5}{\the##6}%
}
\let\pgf@nlt@curveto\pgf@lt@curveto}}% fix me: 0/0 cases and occasional
% dimension too large errors (what's the cause?)
